PIRLNav: Pretraining with Imitation and RL Finetuning for ObjectNav

We study ObjectGoal Navigation -- where a virtual robot situated in a new environment is asked to navigate to an object. Prior work has shown that imitation learning (IL) using behavior cloning (BC) on a dataset of human demonstrations achieves promising results. However, this has limitations -- 1) BC policies generalize poorly to new states, since the training mimics actions not their consequences, and 2) collecting demonstrations is expensive. On the other hand, reinforcement learning (RL) is trivially scalable, but requires careful reward engineering to achieve desirable behavior. We present PIRLNav, a two-stage learning scheme for BC pretraining on human demonstrations followed by RL-finetuning. This leads to a policy that achieves a success rate of $65.0\%$ on ObjectNav ($+5.0\%$ absolute over previous state-of-the-art). Using this BC$\rightarrow$RL training recipe, we present a rigorous empirical analysis of design choices. First, we investigate whether human demonstrations can be replaced with `free' (automatically generated) sources of demonstrations, e.g. shortest paths (SP) or task-agnostic frontier exploration (FE) trajectories. We find that BC$\rightarrow$RL on human demonstrations outperforms BC$\rightarrow$RL on SP and FE trajectories, even when controlled for same BC-pretraining success on train, and even on a subset of val episodes where BC-pretraining success favors the SP or FE policies. Next, we study how RL-finetuning performance scales with the size of the BC pretraining dataset. We find that as we increase the size of BC-pretraining dataset and get to high BC accuracies, improvements from RL-finetuning are smaller, and that $90\%$ of the performance of our best BC$\rightarrow$RL policy can be achieved with less than half the number of BC demonstrations. Finally, we analyze failure modes of our ObjectNav policies, and present guidelines for further improving them.

==> sections/main/challenge_results.tex <==
\section{ObjectNav Challenge 2022}
\label{sec:challenge_results}

\begin{table} %[h!]
    \centering
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{@{}cllrrcrr@{}}
            \toprule
            & & & \multicolumn{2}{c}{\textsc{test-std}} & & \multicolumn{2}{c}{\textsc{test-challenge}} \\
            \cmidrule{4-5} \cmidrule{7-8}
            & & Method & Success $(\mathbf{\uparrow})$ & SPL $(\mathbf{\uparrow})$
                & & Success $(\mathbf{\uparrow})$ & SPL $(\mathbf{\uparrow})$ \\
            \midrule
            %\multirow{3}{*}{\rotatebox[origin=c]{90}{{\footnotesize \textsc{New Inits.}}} $\begin{dcases} \\ \\ \\ \end{dcases}$}
            \\[-10pt]
            & \rownumber & ByteBOT
                & $\mathbf{68.0\%}$ & $\mathbf{37.0\%}$
                & & $64.0\%$ & $\mathbf{35.0\%}$ \\
            & \rownumber & Stretch
                & $60.0\%$ & $34.0\%$
                & & $56.0\%$ & $29.0\%$ \\
            & \rownumber & GoodSeed (ProcTHOR-Large)
                & $54.0\%$ & $32.0\%$
                & & - & - \\
            & \rownumber & Populus A.
                & $66.0\%$ & $32.0\%$
                & & $60.0\%$ & $30.0\%$ \\
            \midrule
            & \rownumber & Ours (BadSeed)
                & $65.0\%$ & $33.0\%$
                & & $\mathbf{65.0}\%$ & $33.0\%$ \\
            \bottomrule
            \end{tabular}
    }
    \vspace{5pt}
    \caption{\objnav results on \textsc{HM3D} \testchallenge and \teststd splits .}
    \label{tab:onav_test_std_challenge}
    % \vspace{-20pt}
\end{table}

In this section, we compare the results of our approach with state-of-the-art approaches on \objnav.
%
In Table. \ref{tab:onav_test_std_challenge} we compare our results with top 4 entries at Habitat \objnav Challenge 2022 \cite{habitat_challenge2022}.
%
Our approach achieves state-of-the-art success rate of $65\%$ on \testchallenge split (row 5, col 3), 
which is $1\%$ better on success and $2\%$ worse on success compared to ByteBOT (row 1, col 3).
%
ByteBOT, a concurrent work, achieves $68\%$ success rate and $37\%$ SPL on \teststd split which is $3\%$ better at success
and $4\%$ better on SPL compared to our approach.
%
Our approach outperforms Stretch \cite{chaplot_neurips20} on both \teststd, $5\%$ better on success and $1\%$ worse on SPL,
and and \testchallenge split, $9\%$ better on success and $4\%$ better on SPL (row 5 \vs row 2).
%
We also compare our to ProcTHOR \cite{procthor}, which achieves $54\%$ success rate and $32\%$ SPL on \teststd split, 
which is $11\%$ worse at success and $1\%$ worse at SPL (row 5 vs row 3).
% 
Another concurrent work on Habitat Challenge 2022 leaderboard, Populus A. (row 4), achieves $66\%$ success and $32\%$ on \teststd split and
$60\%$ success and $30\%$ SPL on \testchallenge split which is $5\%$ worse on success and $3\%$ worse on SPL on \testchallenge split.
% 
\TODO{compress this section}



==> sections/main/questions.tex <==
% \vspace{-15pt}
\section{Questions}
\label{sec:questions}


\begin{itemize}
    \item Describe RL Finetuning Strategy
    \item \question{Is there a lower bound on IL performance on train that you need to achieve to be able successfully RL finetune?} \\
    \answer{Looks like it}
    
    \item \question{Does having a "good" and "very good" IL baseline make a difference during fine-tuning? or do they eventually converge at the same point?} \\
    \answer{This doesn't seem to be the case. A IL-HD policy with $27\%$ val success achieves ${\sim}$similar val success after RL finetuning compared to a IL-HD policy with $54\%$ val success rate.}
    \\
    \ad{How many human demonstrations do you need to IL on to then do well after RL-finetuning? A $54\%$ IL-HD policy gets to the same RL-FT val success as $27\%$. A $0\%$ IL-HD policy probably gets to $0\%$ RL-FT success (right?). So you've identified the two zero gradient regions of a sigmoid ($> 27\%$ and $< 5\%$(?)). Sample this space more densely -- RL-FT with a few different IL-HD points between $0\%$ and $27\%$ -- and scatter plot IL-HD val success vs. RL-FT val success.}
    \\
    \db{Agreed with Abhishek. Let's take our success-vs-number-of-demos plot from Habitat-Web. It kept going up so we kept collecting more data. But let's add to that figure IL->RL offshoots starting from various points on the x-axis. We are claiming that from 27-54, all such IL->RL offshoots converge to the same point. What about 0-27? Where does it stop converging? Also, let's make a claim in this paper that large parts of Habitat-Web data collection may have been unnecessary if annotations are available to do IL->RL finetuning.}
    
    \item \question{Does it matter if the pretrained policy was trained on human demonstrations?} \\
    \answer{Yes, when comparing HD with SP demonstrations we can show that HD demonstrations matter more pretraining for RL finetuning.}
    \\
    \ad{How many SP demos are equivalent to one HD demo? Both during IL and after RL-FT}\\
    \db{People will want to know why. So we have to have a hypothesis.}\\ 
    
    \item \question{Will we get similar performance after fine-tuning if we have a policy that was trained on shortest paths, or trained on demonstrations generated using a frontier exploration strategy, or human demonstrations?} \\
    \answer{No, when comparing results from RL-FT after IL-SP and IL-HD}
    \item \question{Does it have to be an IL pretrained policy? can we not use a policy network from RL policy and discard critic's head?} \\
    \answer{It works irrespective of pretraining objective used, if we discard the critic in case of RL pretraining. Supporting experiments come from ZSON rebuttal.} \\
    \ram{Seems intuitive, does this question and answer add any value to our project?} \\
    \db{It seems to distract a little. Perhaps this can be a final experiment in the end where we say "okay, everything we have analyzed so far used demos; what if we don't have any demos and still want to do RL. RL-from scratch doesn't work. But as ZSON paper has shown maybe we can go from ImageNav to ObjectNav"} \\
    \ram{After thinking more about it, this doesn't seem to add value to our claims. We will be focusing more on demonstrations and not on the RL-FT regime. I think it's fine to exclude this.}
    
    \item \question{Does entropy of IL policy explain better performance during RL-FT?} \\
    \answer{..}
    \item \question{On a SP-favoring or FE-favoring val split (val success for IL-SP or IL-FE > IL-HD) does RL-FT flips the trend on val split?} \\
    \answer{Yes, it does.}
    \item \question{Does RL-FT overwrite IL policy behavior?} \\
    \answer{For IL-SP, it looks like RL-FT overwrites the SP behavior learnt during IL. This is likely not the case for IL-HD, there's some forgetting but looks like IL-HD policy behavior is retained after RL-FT. What about IL-FE?}
    \item \question{If RL-FT overwrites IL policy behavior, what are the behavior it overwrites? Can we quantify it?} \\
    \answer{.....}
    \item \question{For IL-HD RL-FT baseline, are the human-like object-search strategies retained after RL-FT? Does RL-FT evaluate that those skills are adding value to solving the task?}
    \answer{.....}
    \item \question{RL-FT with sparse reward leads to emergence of exploration for IL-SP?} \\
    \answer{For IL-SP checkpoint with ${\sim}30\%$ train success, RL-FT leads to policy learning exploration skills with sparse reward.}
    \\
    \ad{What happens when we do RL-FT for IL-SP below 30\% success?} \\
    \ad{When we compare IL-HD and IL-SP success on the training set, are we using the same set of training set episodes for evaluation?} \\ 
    \ram{We are using a randomly sampled set of 4k episodes from same training split for evaluation} \\
    \item \question{What is the minimum number of human demonstrations we need to get a RL-FT policy with SOTA success rate?} \\
    \answer{Our IL-HD policy trained for 4 epochs vs 20 epochs achieves ${\sim}$\ad{similar} success rate after RL-FT. This tells us about the total experience required to enable successful RL-FT but not about number of demonstrations.}
    \item \question{Do RL-FT SP and FE policies learn to exploit semantic priors?} \\
    \answer{.....}
    \item \question{Collecting FE data is free. Do we outperform HD by collecting more than 70k FE demos?} \\
    \answer{.....}
    \item \question{Which policy is better at semantic navigation to goal objects?} \\
    \answer{.....}
    \item \question{Analysis of failure and success episodes of HD-Best and HD-20k to show they are two different policies.} \\
    \answer{.......}
    % \item \question{Which policy is better at zero-shot generalization to new objects? If we use CLIP text encoder as goal embedding and query HD, FE and SP policies for "new objects" which one generalizes better?} \\
    % \answer{......} \\
    % \ram{I expect HD to better because it learns semantic navigation "skills" and this might help it generalize well to new objects. Thoughts?}
    \item \question{For FE why don't we write down a FE reward and use that for RL-FT? Does that work better?} \\
    \answer{......}
    
    
\end{itemize}

==> sections/rebuttal/rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% \input{imports}
% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% % some bib space saving hacks
% \usepackage{biblatex}
% \addbibresource{strings.bib}
% \addbibresource{main.bib}
% \renewcommand*{\bibfont}{\footnotesize}


% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% % \usepackage[pagebackref,breaklinks,colorlinks,bookmarks=false]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\cvprPaperID{3969} % *** Enter the CVPR Paper ID here
% \def\confName{CVPR}
% \def\confYear{2023}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{PIRLNav: Pretraining with Imitation and RL Finetuning for \objnav}

% \maketitle
% \thispagestyle{empty}
% \appendix

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW

% \input{sections/rebuttal/rebuttal_content}


% %%%%%%%%% REFERENCES
% \begingroup
% % \bibliographystyle{ieeetr}
% % \biboptions{sort&compress}
% % \bibliography{strings,main}
% \setlength\bibitemsep{0pt}
% \newrefcontext[labelprefix=A]
% \printbibliography[heading=none]
% \endgroup


% \end{document}


==> sections/rebuttal/rebuttal_content.tex <==
\noindent We thank reviewers for their feedback!
We are happy that they found our improvements on ObjectNav substantial (\Rtwo{},\Rthree{}),
% 
our IL $\rightarrow$ RL scaling experiments useful (\Rtwo{}),
% 
our ablation study and analysis of failure modes extensive (\Rone{},\Rtwo{}),
% 
the comparisons across different demonstration data sources interesting (\Rtwo{}),
%  (\Rone, \Rtwo{}) and learning rate schedule interesting (\Rtwo{}),
and our paper well-written (\Rone, \Rthree{}).
% 
We address specific comments below and will incorporate all feedback.

\vspace{2pt}
\xhdr{\Rtwo{} \Rone{}: RL experiments with more seeds.} 
% 
As requested, we repeated each RL experiment from Tab. 2, 3 and Fig. 5 with 2 additional seeds.
% 
These results (mean and standard dev across 3 seeds) are in
in Tab.~\ref{tab:rl_ft_comparison},
\ref{tab:rl_ft_ablations_app}, \ref{tab:rl_main_comparison}.
% 
% \cref{tab:rl_ft_comparison} compares PIRLNav with VPT's RL-finetuning approach.
% 
% \cref{tab:rl_ft_ablations_app} ablates the different learning phases when RL-finetuning with PIRLNav.
% 
% Finally, \cref{tab:rl_main_comparison} presents RL-finetuning performance on HM3D \textsc{VAL} 
%when using behavior cloned (BC) checkpoints with equal training success
% on Shortest Path (SP), Frontier Exploration (FE), and Human Demonstrations (HD) respectively.
% 
All trends and findings remain unchanged from the paper. 
Variance across seeds is generally low; consistent with prior findings \cite{wijmans2020train}. 
We will add this to the paper; we hope 
this alleviates any concerns and the reviewers will increase their scores.
% 
% \TODO{add a note about large-scale navigation training trends are in general stable and cite a reference}

\begin{table}[h]
    \centering
    \resizebox{0.30\textwidth}{!}{
        \begin{tabular}{@{}lrr@{}}
            \toprule
            Method & Success $(\mathbf{\uparrow})$ & SPL $(\mathbf{\uparrow})$ \\
            \midrule
            \rownumber BC                                           & $52.0$ & $20.6$ \\
            \rownumber BC$\rightarrow$RL-FT w/ VPT     & $59.7$ {\scriptsize $\pm0.70$} & $\mathbf{28.6}$ {\scriptsize $\pm0.89$} \\
            \midrule
            \rownumber PIRLNav (Ours)                                & $\mathbf{61.9}$ {\scriptsize $\pm0.47$} & $27.9$ {\scriptsize $\pm0.56$}\\
            \bottomrule
            \end{tabular}
    }
    \vspace{2pt}
    \caption{\small Comparison with VPT on HM3D \textsc{val}.
    %~\cite{ramakrishnan_arxiv20,yadav2022habitat}.
    }
    \label{tab:rl_ft_comparison}
    \vspace{-8pt}
\end{table}

\begin{table}[h]
    \centering
    \resizebox{0.95\columnwidth}{!}{
        \begin{tabular}{@{}lrr@{}}
            \toprule
            Method & Success $(\mathbf{\uparrow})$ & SPL $(\mathbf{\uparrow})$ \\
            \midrule
            \rownumber BC                                           & $52.0$ & $20.6$ \\
            \rownumber BC$\rightarrow$RL-FT                                        & $53.6$ {\scriptsize $\pm1.01$} & $\mathbf{28.6}$ {\scriptsize $\pm0.50$}  \\
            \rownumber BC$\rightarrow$RL-FT (+ Critic Learning)                            & $56.7$ {\scriptsize $\pm0.93$} & $27.7$ {\scriptsize $\pm0.82$}\\
            \rownumber BC$\rightarrow$RL-FT (+ Critic Learning, Critic Decay)              & $59.4$ {\scriptsize $\pm0.42$} & $26.9$ {\scriptsize $\pm0.38$} \\
            \rownumber BC$\rightarrow$RL-FT (+ Critic Learning, Actor Warmup)              & $58.2$ {\scriptsize $\pm0.55$} & $26.7$ {\scriptsize $\pm0.69$}\\
            \midrule
            %\rownumber Ours                                         & $\mathbf{62.2}\%$ & $28.7\%$ \\
            \rownumber PIRLNav                                     & $\mathbf{61.9}$ {\scriptsize $\pm0.47$} & $27.9$ {\scriptsize $\pm0.56$} \\
            \bottomrule
            \end{tabular}
    }
    \vspace{2pt}
    \caption{\small RL-finetuning ablations on HM3D \textsc{val}} %~\cite{ramakrishnan_arxiv20,yadav2022habitat}.}
    \label{tab:rl_ft_ablations_app}
    \vspace{-8pt}
\end{table}

\begin{table}[h]
    \centering
    \resizebox{0.8\columnwidth}{!}{
        \begin{tabular}{@{}lrr@{}}
            \toprule
            Demo Source & \textsc{TRAIN} Success $(\mathbf{\uparrow})$ & \textsc{VAL} Success $(\mathbf{\uparrow})$ \\
            \midrule
            \rownumber SP                               & $93.5$ {\scriptsize $\pm0.24$}            & $42.9$  {\scriptsize $\pm0.53$} \\
            \rownumber FE                               & $66.1$ {\scriptsize $\pm0.12$}            & $51.5$  {\scriptsize $\pm0.51$} \\
            \rownumber HD                               & $91.1$ {\scriptsize $\pm0.53$}            & $\mathbf{66.7}$  {\scriptsize $\pm0.54$}\\
            \bottomrule
            \end{tabular}
    }
    \vspace{2pt}
    \caption{\small RL finetuning performance on HM3D TRAIN and VAL after
    BC on shortest paths (SP), frontier exploration (FE), or human demonstrations (HD) with equal BC training success = $48\%$.}
    \label{tab:rl_main_comparison}
    \vspace{-3pt}
\end{table}

\xhdr{\Rone{}: How important is SPL vs Success?}
% \cref{tab:rl_ft_comparison} shows comparison of VPT's RL-Finetuning regime with PIRLNav across 3 training seeds. PIRLNav achieves $61.9\%$ success rate and $27.9\%$ SPL, an improvement of $2.2\%$ on success and $0.7\%$ worse on SPL.
We focus on success because prior work [14, 17] %\cite{objectnav_tech_report}
has argued that SPL is ill-posed for \objnav in unseen environments,
since it penalizes exploration or any deviation from the shortest path 
(which is infeasible to follow in a new house). This makes our improvements more significant. 
% 
%Without a map, following the shortest path to find a goal object in a new environment is not possible.
% if the agent is not following a path
% close to the shortest path it would achieve poor SPL.


% \xhdr{\Rtwo{}: Update reference of IL Learning (IL) to Behavior Cloning (BC).}
% \TODO{Merge this with the point on discussion of IL approaches. Say that we agree that the 
% focus of this paper is on BC (not IL broadly) and that we will change all references of `IL' in
% experiments to `BC'.}
% Thanks for pointing this out, we will update the references in the paper.

\xhdr{\Rtwo{}: Update IL reference to BC.} Thank you! 
We agree with the reviewer and will change the text. 
%that the focus of this paper is on Behavior Cloning (BC), and not Imitation Learning (IL) broadly. We will change references of `IL' to `BC'.

\xhdr{\Rtwo{}: Discussion of other IL methods.}
%
We agree and will add an expanded discussion to the text. To be clear, we use 
behavior cloning (BC) in our experiments 
%BC for pretraining was motivated by results 
to be consistent with and compare to prior state-of-art in ObjectNav[1]. %\cite{ramrakhya2022}. 
that used BC on Human Demonstrations (HD). % and achieved state-of-the-art results on \objnav.
%
It is not clear how to use any alternative IL method in our setting. DAgger requires access to a queryable expert during training which is not feasible for HD. 
%
And no prior work has scaled 
%We are also unaware of any work that applies 
Inverse Reinforcement Learning (IRL) to complex embodied tasks with high dimensional inputs like \objnav. 
%Testing the feasibility of these methods is beyond the scope of this paper. 

%\TODO{Interative imitation learning paper shows results with BC+GAIL in Playhouse environment so a reviewer might say that there is some evidence of using IRL for embodied task. [Erik] It's also not very effective, worse than just BC without auxiliary losses, and they abandoned that direction in the next paper: https://arxiv.org/abs/2112.03763}

\xhdr{\Rthree{}: Combining IL and RL is not very novel.}
% 
% We disagree.
% 
We are unaware of prior work that has combined BC and RL for \objnav. 
% 
We believe this is because combining the two effectively is challenging.
% 
In addition,
% we would like to point out that our RL-Finetuning strategy is not our only contribution.
we also present an empirical study of design choices
in our proposed BC$\rightarrow$RL training recipe, as well as an
analysis of failure modes.

\xhdr{\Rone{}: Clarification about baselines in Tab.~3.}
Baselines in Tab.~3 use different policy architectures and training methods.
%
All baselines train on HM3D-Semantics v0.1, only ProcTHOR pretrains
on ProcTHOR-10k before finetuning on HM3D.
%
Details for published methods can be found in the papers cited in the table.
%Stretch~\cite{chaplot_neurips20} uses a semantic mapping and planning approach trained on HM3D-Semantics v0.1. ProcTHOR-Large~\cite{procthor} trains the EmbCLIP~\cite{khandelwal2021simple} policy using RL on $10k$ procedurally generated environments and finetunes it on HM3D-Semantics v0.1. Habitat-Web uses a policy architecture with RGBD+Semantic segmentation input and learns the policy using BC on $77k$ HD collected on HM3D-Semantics v0.1. DD-PPO trains a policy that takes RGBD input using RL with dense rewards on HM3D-Semantics v0.1. 
`ByteBOT' and `Populus. A' are two unpublished entries from the challenge leaderboard.

\xhdr{\Rtwo{}: Suggestions on LR schedule usage.}
% 
We monitor the critic loss during training, and 
the choice of freezing the actor for $8M$ steps
was based on the convergence of the critic. 
%
We also increased the length of the actor warm-up phase
if we saw a large spike in critic loss.
% 
Will include this.

%\TODO{Thoughts on what else to add here? The schedule is mostly based on a simple hyperparameter sweep and looking at training plots}

\xhdr{\Rtwo{}: Behaviors learned from human demonstrations.}
Prior work [1] showed imitating human \objnav demonstrations  leads to agents learning semantic exploration behaviors, \eg `peeking' into rooms to determine their type.
% 
We find that agents with higher IL success rates demonstrate \emph{more} of such behavior, and also lead to increased RL-finetuned performance. We will add this to the paper. 
% \ie the time spent by these agents in semantically relevant room type for each goal object is higher compared to agents trained with RL. 
% We hypothesize that this provide additional priors about semantics, which is absent from FE design, when searching for objects which leads to improved performance on \objnav. \TODO{Anyone has better suggestions to answer this question?}

\xhdr{\Rone{}: Why do RL-finetuning improvements diminish with IL dataset size?}
% 
%As we increase the size of of the IL pretraining dataset, the improvements from RL-finetuning decrease. \Eg at 20k IL demonstrations, the IL$\rightarrow$RL improvement is 10.1$\%$ success, while at 77k IL demonstrations, the improvement is 6.3$\%$.
% This is expected.
% 
Simply because the room for improvement decreases -- 
IL-pretraining accuracies
go up with IL dataset size (\eg $52.0\%$ at 20k and $64.1\%$ at 77k)
and the RL-finetuning success is upper-bounded
by 100$\%$.
% 
%Nevertheless, IL pretrained policies provide a reasonable starting
%point for `bootstrapping' RL and make the optimization easier
%than learning from scratch. In fact, we show that IL
%pretraining even unlocks RL with sparse rewards for \objnav.


\xhdr{\Rtwo{}: Comparison with alternative RL finetuning methods.}
As a reminder, we compare with a relative entropy term based RL-Finteuning method in Tab. 1 of the paper (shown in~\cref{tab:rl_ft_comparison}). Further research is needed to apply other methods to \objnav (see Appendix A discussion).

\xhdr{\Rtwo{}: What is the equation (curve-fit) in Fig 6?}
This curve predicts the performance on FE dataset-sizes $\geq$ $75$k. We find that for IL-FE, performance plateaus around $75$k as opposed to going up further as one might expect. For comparison, [1] fitted a curve using $35$k human demonstrations and found it predicts performance up to $75$k well.

%The curve fit in Fig. 6 is the equation of a linear model fitted on the training performance of IL-FE baseline with respect to dataset size to plot the expected training performance. 

\xhdr{\Rtwo{}: Were policies fine-tuned on test?} No, only on  HM3D \textsc{TRAIN}.

\xhdr{\Rone{}: Add absolute IL performance in Fig. 1.} Will do.

\xhdr{\Rtwo{}: Fig. 1 not referred in text.} Thanks! Will update.


==> space_saver.tex <==
% A collection of dubious space saving macros
%\setlength{\parindent}{0cm}
%\parskip=2pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{1} % only use this one in emergencies

%Section spacing
\newcommand{\csection}[1]{
    \vspace{-0.08in}
    \section{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsection}[1]{
    \vspace{-0.08in}
    \subsection{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsubsection}[1]{
    \vspace{-0.06in}
    \subsubsection{#1}
    \vspace{-0.05in}
}


%caption/figure spacing
\setlength{\floatsep}{1ex plus 0ex minus 0.5ex}
%\setlength{\textfloatsep}{0ex plus 0ex minus 0ex}
%\setlength{\abovecaptionskip}{0ex plus 0ex minus 0ex}
\setlength{\belowcaptionskip}{0ex plus 0ex minus 0.5ex}
